Infrastructure-less UWB-based Active Relative Localization

In multi-robot systems, relative localization between platforms plays a crucial role in many tasks, such as leader following, target tracking, or cooperative maneuvering. State of the Art (SotA) approaches either rely on infrastructure-based or on infrastructure-less setups. The former typically achieve high localization accuracy but require fixed external structures. The latter provide more flexibility, however, most of the works use cameras or lidars that require Line-of-Sight (LoS) to operate. Ultra Wide Band (UWB) devices are emerging as a viable alternative to build infrastructure-less solutions that do not require LoS. These approaches directly deploy the UWB sensors on the robots. However, they require that at least one of the platforms is static, limiting the advantages of an infrastructure-less setup. In this work, we remove this constraint and introduce an active method for infrastructure-less relative localization. Our approach allows the robot to adapt its position to minimize the relative localization error of the other platform. To this aim, we first design a specialized anchor placement for the active localization task. Then, we propose a novel UWB Relative Localization Loss that adapts the Geometric Dilution Of Precision metric to the infrastructure-less scenario. Lastly, we leverage this loss function to train an active Deep Reinforcement Learning-based controller for UWB relative localization. An extensive simulation campaign and real-world experiments validate our method, showing up to a 60% reduction of the localization error compared to current SotA approaches.

==> Acknoledgment/Acknoledgment.tex <==
\section{Acknowledgment}
This work was supported in
part by the Italian Ministry of University and Research (MUR) under
Grant PRIN 2022P3JY7N, funded by the European Union - Next Generation EU.

==> Methodology/hyper.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.3}
\caption{Hyperparameters and settings}
\label{table:hyper}
\centering
\begin{tabular}{cc}
\hline
\textbf{Hyperparameter} & \textbf{Value} \\
\hline
Gain parameter $\alpha$ & $\left[0.6, 1.4\right]$ \\
Time delay $\delta$ & $\left[0, 50\right]$ ms\\
Sampling time $t_s$ & $0.05$ s\\
Nominal mass $m_0$ & $1$ kg\\
Reward exponent $\beta$ & $1/3$ \\
Reward coefficients $k_v, k_u$ & $0.4$ \\
Reward constant $c$ & $10$ \\
Desired set-point $y_{r}$ & $\left[75\; 0\; 0 \right]^T$ cm \\
Min. allowed distance $y_{m}$ & $40$ cm \\
Noise std.\ dev. $\sigma_w$ & $0.3$ cm \\
Target spawn std.\ dev. $\sigma_s$ & $10$ cm \\
Target traj. amplitude $A_x, A_y, A_z $ & $\left[1, 30\right]$ m \\
Target traj. frequency $f_x, f_y, f_z$ & $\left[0.002, 0.2\right]$ Hz \\
Target traj. phase $\phi_x, \phi_y, \phi_z$ & $\left[0, 2\pi\right]$ \\
Number of agents & $8$ \\
Learning rate & $0.0003$ \\
Batch size & $256$ \\
Max. episode length & $40$ s \\
Replay buffer size & $1,000,000$ samples \\
Angular velocities  $\omega$ saturation & $\left[-4, 4\right]$ rad/s \\
Thrust increment $\lambda$ saturation & $\left[-20, 20\right]$ N/s \\
Observation sequence length $H$ & $15$ steps\\
%Network update interval & $1$ step \\
Discount factor $\gamma$ & $0.99$ \\
\hline
\end{tabular}
\vspace{-1mm}
\end{table}

==> Preliminary/Robot_Dynamic_Model.tex <==
% \subsection{Robot Dynamic Model}\label{sec:Robot Dynamic Model}
% % \textcolor{green}{Valerio
% % bisogna parlare del fatto che non assumiamo incertezze sul robot?
% % }

% % Apprendere una politica di controllo basata su un approccio di RL richiede un'ambiente sicuro dove poter testare e trainare l'algoritmo, pertanto l'addestramento è stato svolto in condizioni simulate.
% % Di conseguenza è stato assunto un modello anche per la piattaforma robotica utilizzata.
% \textcolor{red}{Gabriele: secondo me questa sezione va spostata come sub sub section della parte di RL nel metodo. Nei paper full RL la mettiamo all'inizio perchè il focus è tutto su RL, ma qua è un pò fuorviante e interrompe il ragionamento senza un vero vantaggio.}

% % Training an RL algorithm needs discretized times, therefore we assumed discretized dynamics for the robot model.

==> Preliminary/Short_range_Measurement_Model.tex <==
\subsection{Short range Measurement Problem}\label{section:hort range Measurement Model}
\textcolor{green}{VALERIO}
% La caratterizzazione del modello di misura dei sensori di ranging è un aspetto ampiamente indagato in ambito misuristico.
% Il modello piu comune e piu adottoato nelle applicazioni che sfruttano sensori UWB è quello basato su un modello gaussiano a media nulla e varianza di 5cm \cite{decawave_dwm1001,Brunacci2023_1}. 
% Questo modello funziona bene nel caso di localizzazione svolta nel modo classico e in LOS, quindi con il tag localizzato allàinterno del poligono identificato dalle ancore.
% Tuttavia, il modello di misura di un sensore di raging, in particolare quello di un UWB, è influenzato in maniera non trascurabile dallàambiente di misura e da ostacoli tra i nodi della rete UWB.
% Inoltre, riprendendo quanto detto in Sezione \ref{sec:Geometrical Dilution of Precision}, una piccolo errore sulla misura influenza profondamente la stima di posizione se il GDOP è alto.
% In questo lavoro il setup di misura è sia influenzato dal GDOP che ha un valore chiaramente piu alto del minimo teorico dato da $2/\sqrt{N_m}$ where $N_m$ is the number of the anchors \cite{Levanon2000}, sia è influenzato dal multipath presente nella stanza di misura. 
% Questa infatti è una stanza stretta e allungata, di circa 10x5 m.
% Infine, un altro aspetto che influenza le performance di misura è la distanza.
% Infatti, come osservato in \cite{Iacono2022} e in \cite{Polonelli2022}, i sensori UWB per misure a corto raggio, dai 10 ai 25 cm, presentano un errore  e una varianza sulla misura di distanza maggiore rispetto a quello che riescono a fornire da 25 cm fino a 5 m.
% Considerando queste codizioni quindi, risultava profondamente sconveniente sfruttare un modello che non modella perfettamente le misure.
% Abbiamo quindi deciso di sfruttare un modello di misura ricavato da misure estratte in situazioni affini a quelle che si verificano nelle applicazioni di infrastructureless-relative localization.
% Il modello scelto è quello proposto da Iacono et al. in \cite{Iacono2022} e si basa su un modello esponenziale:
% \begin{equation}
%     f_e(d)=c_1e^{k_1d}
% \end{equation}
% dove $d$ è la distanza di misura e $c_1$ e $k_1$  sono due paramtri con valore rispettivamente 0.51 e −3.152 1/m.


Characterization of the measurement model of ranging sensors is a widely investigated aspect of the measurement field.
The most common and widely adopted model in applications exploiting UWB sensors is the one based on a Gaussian model with zero mean and {\color{blue}standard deviation} of 5 cm \cite{decawave_dwm1001,Brunacci2023_1,Alavi2006}. 
This model works well in the case of localization performed in the classical mode and in LOS, thus with the tag localized within the polygon identified by the anchors.
However, the measurement model of a raging sensor, especially for UWB sensors, is affected in a nontrivial way by the measurement environment and by obstacles between the nodes of the UWB network (NLOS condition).
Moreover, as stated in in Section \ref{sec:Geometrical Dilution of Precision}, a small error in the measurement profoundly affects the position estimation if the GDOP is high.
In this work, the measurement setup is affected by the GDOP, which has a value clearly higher than the theoretical minimum given by $2/\sqrt{N_m}$ where $N_m$ is the number of the anchors \cite{Levanon2000}, and is affected also by the multipath present in the measurement room. 
The experiment room is narrow and elongated, about 10x5 m. \textcolor{red}{Gabriele: è necessaria questa parte così approfondita? Che messaggio/concetto preliminare vogliamo trasmettere? Che il GDOP nel nostro caso è un problema perchè siamo fuori dalle ancore e in NLOS? non basta dire una/due frasi? Da come inizia la sotto sezione sembra che stiamo per dare un modello di misura short range, ma ne paragrafo semplicemente elenchiamo i problemi...}
{\color{Green}
Valerio: questa parte era stata fatta per definire il modello esponenziale di misura che abbiamo adottato nella loss. Per questo sembra porti proprio a quello. Ora il modello viene definito nella sezione della Loss stessa. 
Il messaggio che vogliamo trasmettere è:
1. il modello di misura calssico che si adotta, ossia quello gaussiano non modella bene il funzionamento dei sensori a corto raggio (fino a 25 cm ci sono errori piu alti di quelli dati da una gassiana a media nulla e varianza 5cm).
2. Queste condizioni sono accentuate da ambienti stretti, come una stanza.
3. visto che siamo fuori dal triangolo, il nostro gdop è alto--> errore sulla stima di posizione alto.

Queste condizioni ci portano a dire che non è conveniente usare per un addestramento un modello che modella non bene le nostre condizioni. (il modello gaussiano funziona bene se si sta dentro al triangolo, ma rimane comunque una semplificiazione.)

Inoltre se usassimo il gdop secco come loss, avremmo il minimo al centro delle ancore.

\\--- Si potrebbe spostare tutto questo nella sezione della loss? Abbreviandolo?---
}


